DSV: An Alignment Validation Loss for Self-supervised Outlier Model Selection

Self-supervised learning (SSL) has proven effective in solving various problems by generating internal supervisory signals. Unsupervised anomaly detection, which faces the high cost of obtaining true labels, is an area that can greatly benefit from SSL. However, recent literature suggests that tuning the hyperparameters (HP) of data augmentation functions is crucial to the success of SSL-based anomaly detection (SSAD), yet a systematic method for doing so remains unknown. In this work, we propose DSV (Discordance and Separability Validation), an unsupervised validation loss to select high-performing detection models with effective augmentation HPs. DSV captures the alignment between an augmentation function and the anomaly-generating mechanism with surrogate losses, which approximate the discordance and separability of test data, respectively. As a result, the evaluation via DSV leads to selecting an effective SSAD model exhibiting better alignment, which results in high detection accuracy. We theoretically derive the degree of approximation conducted by the surrogate losses and empirically show that DSV outperforms a wide range of baselines on 21 real-world tasks.

==> 050expres.tex <==
% \section{Experimental Results}

% We answer to the following questions through experiments on real datasets:
% \begin{enumerate}
%     \item[Q1.] \textbf{Performance.}
%         Are the models selected by \method better than those selected by baseline measures for unsupervised model selection?
%         Is the improvement statistically significant across different tasks and datasets? 
%     \item[Q2.] \textbf{Ablation study.}
%         Are the two main components of \method for the discordance and separability, respectively, both meaningful to performance? 
%     \item[Q3.] \textbf{Case studies.}
%         How does \method work on individual cases with respect to the distribution of embedding vectors or the change of AUC?
% \end{enumerate}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.7\textwidth]{paper/figures/ablation/legend.png}

%     \vspace{-2mm}
%     \includegraphics[width=\textwidth]{paper/figures/ablation/cutpaste-1.png}

%     \vspace{-2mm}
%     \includegraphics[width=\textwidth]{paper/figures/ablation/cutpaste-2.png}
%     \caption{
%         Ablation study to compare $\scaledLoss$, $\covLoss$, and $\finalLoss$ on 21 different detection tasks and on average when $\augFunc=\textrm{CutPaste}$.
%         The average AUC is similar between the three models, but \method shows a dramatic improvement over the two baselines in a few cases, such as tasks $T_2$ (both fail), $T_4$ ($\covLoss$ fails), and $T_{14}$ ($\scaledLoss$ fails).
%     }
% \vspaceBelowLargeFigureCaption
% \end{figure}

% \subsection{Detection Performance (Q1)}

% Table \ref{tab:overall-accuracy} shows the average AUC and rank of various approaches on 21 different tasks.
% Due to the lack of space, we include the full results on individual tasks on the supplementary material.
% \method achieves the best performance in either AUC and rank on 6 out of the 8 cases, and the second-best even on the remaining two cases.
% MC and HITS perform relatively well compared to the other approaches, as they were suggested in a recent work, but their performances are not reliable across different augmentation functions and different tasks.

% In Figure \ref{fig:wilcoxon}, we run statistical tests to see if the differences between models are statistically significant.
% We run the Wilcoxon signed rank test \cite{Groggel00Stats}, which has been widely used for a statistical test between different models \cite{yoo2022role}.
% Each number in the $(i, j)$-th cell of the figure represents the $p$-value comparing models $i$ and $j$, and it represents model $i$ is significantly better than model $j$ if the $p$-value is smaller than $0.05$.
% The figure shows that \method is significantly better than all of the other approaches, demonstrating its superiority on UOMS.

% \subsection{Ablation Studies (Q2)}

% \subsection{Case Studies (Q3)}

% In Fig. \ref{fig:embeddings}, we visualize embedding vectors learned on the Carpet object in MVTec AD, when $\augFunc = \textrm{CutOut}$.
% The three cases correspond to CutOut with different patch sizes, which are $0.00004$, $0.00128$, and $0.04$, respectively.
% In Fig. \ref{fig:embeddings-2}, which shows the smallest $\finalLoss$, test anomalies $\smash{\testEmbA}$ are located in between $\trnEmb$ and $\augEmb$.
% Although some of $\smash{\testEmbA}$ are mixed with $\smash{\testEmbN}$, the AUC is high as $0.815$.
% On the other hand, in Figs. \ref{fig:embeddings-1} and \ref{fig:embeddings-3}, the AUC is lower than even a random guess, while $\finalLoss$ is large.
% In Fig. \ref{fig:embeddings-1}, since the amount of augmentation is too small, test normal data are anomalies are mixed without separation.
% In Fig. \ref{fig:embeddings-3}, since the amount of augmentation is too large, test anomalies are separated from even test augmented data, exhibiting severe misalignment.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.85\textwidth]{paper/figures/emb-cutout/legend.png}
%     \vspace{-1mm}
    
%     \begin{subfigure}{0.32\textwidth}
%         \includegraphics[width=\textwidth]{paper/figures/emb-cutout/carpet-1.png}
%         \caption{Patch size: $0.00004$}
%         \label{fig:embeddings-1}
%     \end{subfigure} \hfill
%     \begin{subfigure}{0.32\textwidth}
%         \includegraphics[width=\textwidth]{paper/figures/emb-cutout/carpet-2.png}
%         \caption{Patch size: $0.00128$}
%         \label{fig:embeddings-2}
%     \end{subfigure} \hfill
%     \begin{subfigure}{0.32\textwidth}
%         \includegraphics[width=\textwidth]{paper/figures/emb-cutout/carpet-3.png}
%         \caption{Patch size: $0.04$}
%         \label{fig:embeddings-3}
%     \end{subfigure}

%     % \vspace{2mm}
%     % \begin{subfigure}{0.32\textwidth}
%     %     \includegraphics[width=\textwidth]{paper/figures/emb-cutpaste/metal_nut-1.png}
%     %     \caption{CutPaste}
%     % \end{subfigure} \hfill
%     % \begin{subfigure}{0.32\textwidth}
%     %     \includegraphics[width=\textwidth]{paper/figures/emb-cutpaste/metal_nut-2.png}
%     %     \caption{CutPaste}
%     % \end{subfigure} \hfill
%     % \begin{subfigure}{0.32\textwidth}
%     %     \includegraphics[width=\textwidth]{paper/figures/emb-cutpaste/metal_nut-3.png}
%     %     \caption{CutPaste}
%     % \end{subfigure}

%     \caption{
%         $t$-SNE visualizations of embeddings with different values of hyperparameters in $\augFunc = \textrm{CutOut}$.
%         The value of $\finalLoss$ is the smallest in (b), where the test anomalies $\smash{\testEmbA}$ are in between $\trnEmb$ and $\augEmb$.
%         The detection fails at (a) and (c) with different types of misalignment, showing larger $\finalLoss$ than in (b).
%     }
% \label{fig:embeddings}
% \vspaceBelowLargeFigureCaption
% \end{figure}


==> 060related.tex <==
% \section{Related Works}

% We introduce related works.

% \paragraph{Unsupervised anomaly detection.}

% Unsupervised anomaly detection is an important problem.

% \paragraph{Self-supervised learning.}

% Self-supervised learning is a cool technique.

% \paragraph{Unsupervised model selection.}

% Unsupervised model selection is super important.


